Empirical Bayes Estimates for a 2-Way Cross-Classified Additive Model

We develop an empirical Bayes procedure for estimating the cell means in an unbalanced, two-way additive model with fixed effects. We employ a hierarchical model, which reflects exchangeability of the effects within treatment and within block but not necessarily between them, as suggested before by Lindley and Smith (1972). The hyperparameters of this hierarchical model, instead of considered fixed, are to be substituted with data-dependent values in such a way that the point risk of the empirical Bayes estimator is small. Our method chooses the hyperparameters by minimizing an unbiased risk estimate and is shown to be asymptotically optimal for the estimation problem defined above. The usual empirical Best Linear Unbiased Predictor (BLUP) is shown to be substantially different from the proposed method in the unbalanced case and therefore performs sub-optimally. Our estimator is implemented through a computationally tractable algorithm that is scalable to work under large designs. The case of missing cell observations is treated as well. We demonstrate the advantages of our method over the BLUP estimator through simulations and in a real data example, where we estimate average nitrate levels in water sources based on their locations and the time of the day.

==> append-balanced.tex <==
\begin{align}
R(\eta, \etahat^{y_{\cdot \cdot}, \lambdaa, \lambdab}) 
&= \frac{1}{rc} E \Big\{  \sum_{i=1}^r \sum_{j=1}^c (   \muhat^{y_{\cdot \cdot}, \lambdaa, \lambdab}+  \alphahat^{y_{\cdot \cdot}, \lambdaa, \lambdab} + \betahat^{y_{\cdot \cdot}, \lambdaa, \lambdab} - m - a_i - b_j  )^2  \Big\} \label{eq:risk-bal}\\
&= \frac{1}{rc} E \Big\{  \sum_{i=1}^r \sum_{j=1}^c (   \mhatls +  c_{\alpha} \ahatls_i + c_{\beta} \bhatls_j - m - a_i - b_j  )^2  \Big\} \\
&= \frac{1}{rc} E \Big\{  \sum_{i=1}^r \sum_{j=1}^c [   (\mhatls - m) +  (c_{\alpha} \ahatls_i - a_i) +  (c_{\beta} \bhatls_j - b_j) ]^2  \Big\} \\
&= \frac{1}{rc} E \Big\{  rc(\mhatls - m)^2 + c \sum_{i=1}^r(c_{\alpha} \ahatls_i - a_i)^2 + r \sum_{j=1}^c(c_{\beta} \bhatls_j - b_j)^2  \Big\} \label{eq:orth} \\
&= E\Big\{  (\mhatls - m)^2  \Big\} + \frac{1}{r} E\Big\{  \sum_{i=1}^r(c_{\alpha} \ahatls_i - a_i)^2 \Big\} + \frac{1}{c} E\Big\{  \sum_{j=1}^c(c_{\beta} \bhatls_j - b_j)^2 \Big\} \label{eq:lin}
\end{align}
where equality \eqref{eq:orth} is due to orthogonality of the vectors corresponding to the three sums-of-squares. %and \eqref{eq:lin} is due to linearity of expectation
Since, marginally, 
\bel{eq:ls-marginal}
\mhatls \sim N(m, \sigma^2 \lambda^2_m),\ \ \ \ \ \ahatls \sim N_r(a, \sigma^2 \Lambda_a),\ \ \ \ \ \bhatls \sim N_c(b, \sigma^2 \Lambda_b), 
\eel
with known $\lambda^2_m, \Lambda_{\alpha}, \Lambda_{\beta}$ (and $\sigma^2$), SURE can be written as the sum of three separate SURE expressions, one for each of the summands in \eqref{eq:orth}. 
Minimizing SURE for $\etahat^{y_{\cdot \cdot}, \lambdaa, \lambdab}$ jointly over $c_{\alpha}, c_{\beta}$ therefore consists of minimizing separately the ``row" term over $c_{\alpha}$ and the ``column" term over $c_{\beta}$. 
%By \eqref{eq:ls-marginal}, 
Each of these is a ``one-way" Gaussian homoscedastic problem, except that the covariance matrices $\Lambda_{\alpha}, \Lambda_{\beta}$ are singular (because main effects are centered). 
This will be taken into account in writing SURE for each, namely, the SURE estimate will have the ``correct" degrees-of-freedom. 

==> balanced-old.tex <==
In this section, we discuss the special case of balanced designs where $K_{ij} = k \rm{ for } 1 \leq i \leq R,  1 \leq j \leq C$. The balanced case can be decoupled into two independent one-way problems and existing EB methods from the one-way ANOVA set-up can be used to efficiently solve this problem. To further explain the case, without loss of generality, we assume $k=1$. We also impose the restriction on model \eqref{eq:model-twoway} that the mean of the row and column effects are both zero. This is a popularly used restriction for estimation in balanced designs (See Ch. 6 of \citealp{sengupta2003linear}). The main effects - general effect, row effect and column effect are identifiable and are denoted by: 
\bel{eq:main-effects} 
m = \mu + \alpha_{\cdot} + \beta_{\cdot},\ \ \ \ a_i = \alpha_i - \alpha_{\cdot},\ \ \ \ b_j = \beta_j - \beta_{\cdot} \ . 
\eel
where $\alpha_{\cdot}$ and $\beta_{\cdot}$ are the mean of the row and column effects respectively. 
%We consider a hierarchical prior structure on $a_i$s and $b_j$s, which results in an EB class of estimators which shrinks towards the grand mean of all the observations. 
The cannonical Least Squares estimates are given by:
\bel{eq:ls-bal}
\mhatls = y_{\cdot \cdot }, \ \ \ \ \ \ahatbls_i = y_{i\cdot} - y_{..} \;, \ \ \ \ \ \bhatbls_i = y_{\cdot j} - y_{..} \;,
\eel
where $y_{..}$ is the over all mean, $y_{\cdot j}=r^{-1}\sum_{i=1}^r y_{ij}$ and  $y_{i \cdot }=c^{-1}\sum_{j=1}^c y_{ij}$. Considering Bayes estimators of $\etab$ centered around the overall grand mean $y_{..}$, we found they are of the following form:
\bel{eq:sure-bs}
\big \{ \etahatsb(y_{\cdot \cdot}, \lambdaa, \lambdab) \big \}_{ij} = \mhatls + c_{\alpha}(\lambdaa) \; \ahatls_i + c_{\beta}(\lambdab) \; \bhatls_j  
\eel
 where $c_{\alpha} := c_{\alpha}(\lambdaa)=\lambdaa/(\lambdaa+\sigma^2/c)$ and $c_{\beta} := c_{\beta}(\lambdab)=\lambdab/(\lambdab+\sigma^2/r)$ are functions involving only $\lambdaa$ and $\lambdab$ respectively (for Proof see Appendix~REF). Thus, the grand mean centered EB estimator in this balanced case can be separated into shrinkage components which solely depend on (a) overall effect (b) row effects (c) column effects. As shown in appendix REF that estimation of each of these three components can be done separately  due to orthogonality of the vectors corresponding to the their sums-of-squares. As such, the risk associated with  \eqref{eq:sure-bs} splits into the following three components which are orthogonal to each other based on sufficiency arguments in the normal model \eqref{eq:model-twoway}:
 \begin{align}
 \begin{split}
 R(\etab, \etahatsb(y_{\cdot \cdot}, \lambdaa, \lambdab)) 
 = & \ex\Big\{  (\mhatls - m)^2  \Big\} \\
 & + r^{-1} \ex \Big\{  \sum_{i=1}^r(c_{\alpha} \ahatls_i - a_i)^2 \Big\} + {c}^{-1} \ex \Big\{  \sum_{j=1}^c(c_{\beta} \bhatls_j - b_j)^2 \Big\}. 
 \end{split}\label{eq:lin}
 \end{align}
Since, marginally, 
\bel{eq:ls-marginal}
\mhatls \sim N(m, \sigma^2 (rc)^{-1} ),\ \ \ \ \ \ahatbls \sim N_r(a, \sigma^2 \Lambda_a),\ \ \ \ \ \bhatbls \sim N_c(b, \sigma^2 \Lambda_b), 
\eel
with known  $\Lambda_{\alpha}, \Lambda_{\beta}$ (and $\sigma^2$). Stein's Unbiased Risk estimate (SURE) of the above risk can be written as the sum of three separate SURE expressions, one for each of the summands in \eqref{eq:lin}. 
Minimizing the SURE over the class of $\etahatsb(y_{\cdot \cdot}, \lambdaa, \lambdab)$ thus does not involve  joint minimization over the two hyper-parameters $c_{\alpha}, c_{\beta}$ but consists of minimizing separately the ``row" term over $c_{\alpha}$ and the ``column" term over $c_{\beta}$. Each of these is a ``one-way" Gaussian homoscedastic problem, except that the covariance matrices $\Lambda_{\alpha}, \Lambda_{\beta}$ are singular because main effects are centered. This can be easily taken into account in writing SURE by following the steps in Section~\ref{sec:missing}. 
\par
The maximum-likelihood estimates for the two-way random-effects, additive model do not have a closed-form solution even for balanced data \citep[see][Ch. 4.7 d.]{searle2009variance}.
%and it is known (for example, by considering the one-way layout, where they do have an easy, closed-form solution) that the MLE for variance components does not take into account the estimation of the fixed effects in determining the degrees-of-freedom. 
The REML estimates  coincide with the positive-part Moments method estimates \citep[][Ch. 4.8]{searle2009variance}, which, in turn, reduce (for known $\sigma^2$) to solving separately two one-way problems involving $\ahatls$ for the rows and $\bhatls$ for the columns. 
These have the usual closed-form solutions and are easily seen to coincide with the SURE solutions. Thus, for balanced data, if we consider linear estimators that shrink towards the overall mean, the hyper-parameters estimated by the REML method match those produced by the SURE methodology.
\par
The independence of $\mhatls, \ahatls, \bhatls$ in the balanced case was not needed for the proof of \eqref{eq:lin}. However, in the unbalanced case, we no longer have the decomposition of the risk into the orthogonal components as in \eqref{eq:lin}, because the {\it Bayes} estimates in this case for $\alphab$ and $\betab$ do not depend on solely $\ahatbls$ and $\bhatbls$ respectively like in the balanced case.  
We can still use shrinakge estimators of the form \eqref{eq:sure-bs} and look for ``optimal" constants $c_{\alpha} = c_{\alpha}(\lambdaa)$ and $c_{\beta} = c_{\beta}(\lambdab)$ in terms of the risk. As such, contrasting the performance of this class of shrinkage estimators with our concerned class $\mathcal{S}[\tau]$ of EB estimators which account for the two-way nature of our concerned problem,  will display the relative efficiency of using one-way methods in the Two-way mean estimation problem. To minimize the criterion in \eqref{eq:lin}  over $\lambdaa$ and $\lambdab$, we separately use the SURE based method of \citet{xie2012sure} for the normal mean vector estimation problem and estimate the shrinkage coefficients
$c_{\alpha}$, $c_{\beta}$ based on  $\bold{\ahatls}$, $\bold{\bhatls}$ respectively. The estimates are:
%By \eqref{eq:lin}, the solution for $c_{\alpha}$ must be optimal for the one-way problem involving only $\ahatls$ (and similarly for $c_{\beta}$ with $\bhatls$), and is asymptotically attained by the SURE estimate of \citet{xie2012sure}. 
\begin{align}\label{eq:xkb-twoway}
\etahat^{\rm{XKB}}_{ij} &= \mhatls + \chat^{\rm{XKB}}_{\alpha} \;\ahatls_i + \chat^{\rm{XKB}}_{\beta} \; \bhatls_j,\ \ \ 1\leq i \leq r,\ 1\leq j \leq c \quad \rm{ where, }\\
\chat^{\rm{XKB}}_{\alpha} &= \argmin_{c_{\alpha} \in [0,1]} \URE \Big\{  \sum_{i=1}^r(c_{\alpha} \ahatls_i - a_i)^2 \Big\}, \\
\chat^{\rm{XKB}}_{\beta} &= \argmin_{c_{\beta}  \in [0,1]} \URE \Big\{  \sum_{j=1}^c(c_{\beta} \bhatls_j - b_j)^2 \Big\}
\end{align}
%E\Big\{  \sum_{j=1}^c(c_{\beta} \bhatls_j - b_j)^2 \Big\}
For uniformly estimating of the above two risk functions, we slightly modify the parametric SURE estimate of \citet{xie2012sure} that shrinks towards the origin to accommodate the covariance structure of the centered random vectors $\ahatls, \bhatls$. We extensively study the performance of this class on estimators denoted by XKB through numerical simulations in Section~\ref{sec:computation}.  As shown in \citet{xie2012sure}, the estimates of $c_{\alpha}$ and $c_{\beta}$ produced by maximum-likelihood empirical Bayes (EBMLE) and Moments-method empirical Bayes (EBMOM) are generally different for heteroscedastic observations and following their theory we know that the SURE used here is asymptotically optimal for the one-way problem and hence for large balanced designs. The decoupling phenomenon seen for estimation in two-way balanced design extends over to the proportional cells model where $K_{ij}=k_{i,1} \cdot k_{j,2}$ for all $(i,j)$ pairs. 
 

==> left-out-proof.tex <==
\bigskip

\noindent {\it Proof of Theorem~\ref{thm:loss-approx}}. \ 
%Denote $SURE(y; \mu, \lambdaa, \lambdab) = SURE(y; \mu, \lambdaa, \lambdab)$ and let $SURE(y; \lambdaa, \lambdab) = SURE(y; 0, \lambdaa, \lambdab)$. 
%Denote also $R_{r,c}(\eta; \mu, \lambdaa, \lambdab) = R_{r,c}(\eta, \etahat^{\mu, \lambdaa, \lambdab})$ and let $R_{r,c}(\eta; \lambdaa, \lambdab) = R_{r,c}(\eta; 0, \lambdaa, \lambdab)$. 
Let $G = M \Vinv$ and $G^2 = G^{\topp}G$. 
Let
\bes
\gamma_{r,c} = \frac{ \max \{K_{ij}: i\leq r, \ j\leq c \} }{ \min \{K_{ij}: i\leq r, \ j\leq c \} }. 
\ees
We denote by $\sigma_k(A)$ the $k$-th largest singular value of a matrix $A$. 
We denote by $\lambda_k(B)$ the $k$-th largest eigenvalue of a square diagonalizable matrix $B$. 

\benu[(a)]
\item Fix $\lambdaa, \lambdab \geq 0$. 
We consider first the case $\mu = 0$ and show that 
\bes
E[ SURE(y; 0, \lambdaa, \lambdab) -  R_{r,c}(\eta; \etahat^{0, \lambdaa, \lambdab})]^2 \to 0 \ \ \text{as } r,c\to \infty.
\ees

\noindent We have
\begin{align}
E[ SURE(y; 0, \lambdaa, \lambdab) -  R_{r,c}(\eta; \etahat^{\mu, \lambdaa, \lambdab})]^2 &= \Var[ SURE(y; 0, \lambdaa, \lambdab) ] = \frac{1}{r^2 c^2} \Var(y^{\topp}G^2y) \notag \\ 
& = \frac{1}{r^2 c^2} \{ 2\tr(G^2MG^2M) + 4\eta^{\topp}G^2MG^2\eta \} \label{eq:var-sure-zero}
\end{align}

Let $W = M^{\frac{1}{2}} \Vinv M^{\frac{1}{2}}$ . 
From $0<M\leq V$ 
%and \eqref{fc:psd-inv}+\eqref{fc:psd-butterfly}, 
 it follows that $W\leq I$, and therefore also $W^2\leq I$. 
Hence 
\begin{align*}
\lambda_1(G^2MG^2) &= \lambda_1(\Vinv M^2 \Vinv M \Vinv M^2 \Vinv) = \lambda_1(\Vinv M^{\frac{3}{2}} W^2 M^{\frac{3}{2}} \Vinv) \\
&\leq \lambda_1(\Vinv M^3 \Vinv) = \lambda_1(M^{-\frac{1}{2}} W M^2 W M^{-\frac{1}{2}}) = \sigma_1^2(M^{-\frac{1}{2}} W M ) \\
&\leq \{ \sigma_1(M^{-\frac{1}{2}}) \sigma_1(W) \sigma_1(M) \}^2 = \{ \lambda_1^{1/2}(\Minv) \lambda_1(W) \lambda_1(M) \}^2 \\
&\leq \lambda_1^2(M) \lambda_1(\Minv) = (\max K_{ij}) / (\min K_{ij})^2 \leq \gamma_{r,c}.
\end{align*}
%where the first inequality uses facts \eqref{fc:psd-inv} and \eqref{fc:psd-butterfly}, and the second inequality uses \eqref{fc:singular-prod}. 
Since $\eta^{\topp} G^2 M G^2 \eta \leq \lambda_1(G^2 M G^2) \|\eta\|^2$, it follows that 
\bes
\eta^{\topp} G^2 M G^2 \eta \leq \gamma_{r,c}\|\eta\|^2.
\ees

\noindent Also, as $W^2\leq I$, 
\begin{align*}
\tr(G^2MG^2M) &= \tr(M^\half G^2 M G^2 M^\half) = \tr(M^\half \Vinv M^2 \Vinv M \Vinv M^2 \Vinv M^\half) \\
&= \tr(M^\half \Vinv M^{\frac{3}{2}} W^2 M^{\frac{3}{2}} \Vinv M^\half) \leq \tr(M^\half \Vinv M^3 \Vinv M^\half) \\
&= \tr(W M^2 W) = \tr(M W^2 M) \leq \tr(M^2) = rc\cdot \max(K_{ij}^{-1})\leq rc
\end{align*}
Hence the RHS of \eqref{eq:var-sure-zero} is no more than $\frac{1}{r^2c^2} \{ 2\tr(M^2) + 4\gamma_{r,c}\|\eta\|^2 \} \to 0$ as $r,c \to \infty$ by the assumptions of the theorem. 

\bigskip 

Now, for arbitrary $\mu \in \R$, we have
\bes
SURE(y; \mu, \lambdaa, \lambdab) = SURE(y; 0, \lambdaa, \lambdab) + \rcinv \mu^2 1^{\topp} G^2 1 - \rcinv 2\mu y^{\topp} G^2 1,
\ees
hence
\begin{align*}
E[ SURE(y; \mu, \lambdaa, \lambdab) -  R_{r,c}(\eta; \etahat^{\mu, \lambdaa, \lambdab})]^2 &= \Var[SURE(y; \mu, \lambdaa, \lambdab)] \\
&\leq 2 \{ \Var[SURE(y; 0, \lambdaa, \lambdab)] + \frac{4}{r^2c^2} \mu^2 \Var(y^{\topp}G^2 1)\}.
\end{align*}
In the last expression, the first term inside the braces was shown above to tend to 0. 
As for the second term, we need to show that $\frac{4\mu^2}{r^2c^2} 1^{\topp} G^2 M G^2 1 \to 0$ as $r,c \to \infty$. 

\noindent Since $\lambda_1(G^2MG^2) \leq \gamma_{r,c}$ as was shown above, it follows that 
\bes
\rcsqinv 1^{\topp} G^2 M G^2 1 \leq \rcsqinv rc \gamma_{r,c} \leq \rcinv \gamma_{r,c} \to 0 \text{ as } r,c \to \infty
\ees
implying that $\frac{4\mu^2}{r^2c^2} 1^{\topp} G^2 M G^2 1 \to 0$ as $r,c \to \infty$ for any $\mu$.

As $\mu$ is bounded, and since all bounds above on terms in \eqref{eq:var-sure-zero} are indpendent of $\lambdaa$ or $\lambdab$, it follwos that $\displaystyle \sup_{|\mu|\leq B, \lambdaa, \lambdab \geq 0} \Var[SURE(y; \mu, \lambdaa, \lambdab)]$ also tends to zero as $r,c \to \infty$. 

\item
%SURE(y; \mu, \lambdaa, \lambdab) - L(\eta, \etahat^{\mu, \lambdaa, \lambdab})
Fix $\lambdaa, \lambdab \geq 0$. 
We consider first the case $\mu = 0$ and show that 
\bes
E [ L(\eta, \etahat^{0, \lambdaa, \lambdab}) - R_{r,c}(\eta; \etahat^{0, \lambdaa, \lambdab}) ]^2 \to 0 \text{ as } r,c\to \infty. 
\ees
For $\etahat = \etahat^{0, \lambdaa, \lambdab}$ we have 
\begin{align*}
L(\eta, \etahat) &= \rcinv (\etahat - \eta)^{\topp}(\etahat - \eta) = \rcinv (y - \eta - Gy)^{\topp} (y - \eta - Gy) \\
&= \rcinv \big\{ (y-\eta)^{\topp}(y-\eta) + y^{\topp}G^2y - 2(y-\eta)^{\topp}Gy \big\} \\
&= \rcinv \big\{ \underbrace{(y-\eta)^{\topp}(y-\eta)}_{Q_1} + \underbrace{y^{\topp}G^2y}_{Q_2} -  \underbrace{2y^{\topp}Gy}_{Q_3} +  \underbrace{2\eta^{\topp}Gy}_{Q_4} \big\}
\end{align*}
hence it suffices to show that for each of the four terms above $E[ \rcinv Q_i - E(\rcinv Q_i) ]^2 = \Var(\rcinv Q_i) \to \infty$ as $r,c \to \infty$. 

$Q_1$: $\rcsqinv \Var[(y-\eta)^{\topp}(y-\eta)] = \rcsqinv 2\tr(M^2) \to 0$ as $r,c \to \infty$. 

$Q_2$: $\rcsqinv \Var(y^{\topp}G^2y) \to 0$ as $r,c \to \infty$ was already shown in the proof of part (a). 

$Q_3$: $4\Var(y^{\topp}Gy) = 2\tr(\Gtil M \Gtil M) + 4\eta^{\topp} \Gtil M \Gtil \eta$, \ \ \ $\Gtil = G + G^{\topp}$.

%\textcolor{white}{$Q_3$:} 
For the second of the two terms on the RHS, as $\Gtil = G + G^{\topp} = M\Vinv + \Vinv M$, 
\bes
\Gtil M \Gtil = \underbrace{M\Vinv M M \Vinv}_{Q_{31}} + \underbrace{M\Vinv M\Vinv M}_{Q_{32}} + \underbrace{\Vinv M M M \Vinv}_{Q_{33}} + \underbrace{\Vinv MM \Vinv M}_{Q_{34}}.
\ees
%\textcolor{white}{$Q_3$:} 
We show that $\rcsqinv |\eta^{\topp} Q_{3i} \eta| \to 0$ as $r,c \to \infty$ for $i=1,...,4$. 

$Q_{31}$: 
Under the assumption of the theorem,
\begin{align*}
\lambda_1(G^2) = \lambda_1(\Vinv M^2 \Vinv) = \lambda_1(M^{-\half}WMWM^{-\half}) &= \sigma_1^2\{ M^{-\half}W M^\half \} \\
&\leq \{ \sigma_1(M^{-\half}) \sigma_1(W) \sigma_1(M^\half) \}^2 \\
&\leq \{ \sigma_1(M^{-\half}) \sigma_1(M^\half) \}^2 = \gamma_{r,c}. 
\end{align*}
%where the first inequality uses fact \eqref{fc:singular-prod}. 
Hence 
\bes
\lambda_1(M\Vinv M M \Vinv) \leq \lambda_1(M)\lambda_1(\Vinv M^2 \Vinv) = \lambda_1(M)\lambda_1(G^2) \leq \lambda_1(G^2)\leq \gamma_{r,c}
\ees
%where we used fact \eqref{fc:psd-eigen-prod} for the first inequality, noting 
and we note that $M\Vinv M M \Vinv$ is indeed diagonalizable as a product of two p.s.d. matrices. %\texttt{[REFERENCE]}. 
Therefore, 
\bes
\rcsqinv | \eta^{\topp} (M\Vinv M M \Vinv) \eta | \leq \rcsqinv \lambda_1(M\Vinv M M \Vinv) \| \eta \|^2 \leq \rcsqinv \gamma_{r,c} \|\eta\|^2 \to 0
\ees
as $r,c \to \infty$. 

$Q_{34}$:
Since $\eta^{\topp} (\Vinv M M \Vinv M) \eta = \eta^{\topp} (M\Vinv M M \Vinv) \eta$, it follows that $\rcsqinv | \eta^{\topp} (\Vinv M M \Vinv M) \eta | \to 0$ as well.

$Q_{32}$:
We have 
\begin{align*}
\lambda_1(M \Vinv M \Vinv M) &\leq \lambda_1(M V^{-2} M) \\
&= \lambda_1\{M^\half (M^\half V^{-2} M^\half) M^\half\} \\
&\leq \lambda_1(\Minv) \lambda_1(M) = \gamma_{r,c}
\end{align*}
where the last inequality is due to
\bes
M^\half V^{-2} M^\half = (M^\half V^{-2} M^\half) \Minv (M^\half V^{-2} M^\half) \leq \lambda_1(\Minv) I.
\ees
Hence, $\rcsqinv \eta^{\topp} (M \Vinv M \Vinv M) \eta \leq \rcsqinv \gamma_{r,c}\|\eta\|^2 \to 0$ as $r,c \to \infty$. 

$Q_{33}$: 
Finally, $\lambda_1(\Vinv M^3 \Vinv) \leq \gamma_{r,c}$ was shown in the proof of part (a) of the theorem, implying
\bes
\rcsqinv \eta^{\topp} \Vinv M^3 \Vinv \eta \leq \rcsqinv \gamma_{r,c} \|\eta\|^2 \to 0 
\ees
as $r,c \to \infty$. 

\bigskip

Now, as for $\tr(\Gtil M \Gtil M)$ we have
\bes
\Gtil M \Gtil M = GMGM + GMG^{\topp}M + G^{\topp}MGM + G^{\topp}MG^{\topp}M
\ees
hence
\bes
\tr(\Gtil M \Gtil M) = 2\tr(GMGM) + 2\tr(GMG^{\topp}M).
\ees
Since
%, using fact \eqref{fc:psd-butterfly}, 
\begin{align*}
\tr(GMGM) = \tr(M\Vinv M^2 \Vinv M) &= \tr(MG^2M) \leq \tr\{ M[\lambda_1(G^2)I]M \} \\
&= \lambda_1(G^2) \tr(M^2) = \gamma_{r,c} \tr(M^2),
\end{align*}
then
\bes
\rcsqinv \tr(GMGM) \leq \rcsqinv \gamma_{r,c} \tr(M^2) \to 0
\ees
as $r,c \to \infty$. 

Also, as $W^2\leq I$, 
\begin{align*}
\tr(GMG^{\topp}M) = \tr(M\Vinv M \Vinv M M) &= \tr(M M^\half \Vinv M \Vinv M^\half M) \\
&=\tr(MW^2M) \leq \tr(M^2)
\end{align*}
and so
\bes
\rcsqinv \tr(GMG^{\topp}M) \leq \rcsqinv \tr(M^2) \to 0
\ees
as $r,c \to \infty$. 

Together, we have 
\bes
\rcsqinv \tr(\Gtil M \Gtil M) \to 0
\ees
as $r,c \to \infty$

We conclude that $\rcsqinv \Var(y^{\topp}Gy) \to 0$ as $r,c \to \infty$.

$Q_4$: $\Var(\eta^{\topp} G y) = \eta^{\topp} GMG^{\topp} \eta$.
Using again the fact that $W^2\leq I$, 
\bes
\lambda_1(GMG^{\topp}) = \lambda_1(M\Vinv M \Vinv M) = \lambda_1(M^\half W^2 M^\half) \leq \lambda_1(M) \leq 1
\ees
and so
\bes
\rcsqinv \eta^{\topp} GMG^{\topp}\eta \leq \rcsqinv \lambda_1(GMG^{\topp}) \| \eta \|^2 \to 0
\ees
as $r,c \to \infty$.

\bigskip

Turning to the case of arbitrary $\mu \in \R$, we first note that
\bel{eq:loss-general-mu}
\begin{aligned}
rc\cdot L(\eta, \etahat^{\mu, \lambdaa, \lambdab}) 
&= (\etahat^{\mu, \lambdaa, \lambdab} - \eta)^{\topp} (\etahat^{\mu, \lambdaa, \lambdab} - \eta) \\
&= (\etahat^{0, \lambdaa, \lambdab} - \eta)^{\topp} (\etahat^{0, \lambdaa, \lambdab} - \eta) + \mu 1^{\topp}G^{\topp}G1\\
&+ 2\mu 1^{\topp}G^{\topp}(I-G)y - 2\mu 1^{\topp}G\eta.
\end{aligned}
\eel
and so
\bes
\begin{aligned}
E [L(\eta, \etahat^{\mu, \lambdaa, \lambdab}) - R(\eta,\etahat^{\mu, \lambdaa, \lambdab})]^2 
&=  \Var[ L(\eta, \etahat^{\mu, \lambdaa, \lambdab}) ]\\
&\leq \rcsqinv \big[ \Var( (\etahat^{0, \lambdaa, \lambdab} - \eta)^{\topp} (\etahat^{0, \lambdaa, \lambdab} - \eta) ) \\
&+ \Var(2\mu 1^{\topp}G^{\topp}(I-G)y) \big]
\end{aligned}
\ees

Now, $\Var( (\etahat^{0, \lambdaa, \lambdab} - \eta)^{\topp} (\etahat^{0, \lambdaa, \lambdab} - \eta) )$ has been just dealt with in the $\mu=0$ case. 
Therefore, it remains to show that
\bes
\mu^2 \rcsqinv \Var(1^{\topp} G^{\topp}(I-G)y) \to 0
\ees
as $r,c \to \infty$. 
Now, 
\begin{align}
\begin{split}
\Var(1^{\topp} G^{\topp}(I-G)y) = 1^{\topp}G^{\topp}(I-G)M(I-G)^{\topp}G1 &\leq \lambda_1(G^{\topp}(I-G)M(I-G)^{\topp}G)1^{\topp}1 \\
&= rc \cdot \lambda_1(G^{\topp}(I-G)M(I-G)^{\topp}G).
\end{split}
\end{align}
Let $L = M^{-\half} (M-GM)\Minv (M-GM)M^{-\half}$ and note that $(M-GM)$ is symmetric. 
Since $M-GM \leq M$, then $M^{-\half}(M-GM)M^{-\half} \leq I$, and by squaring we get that $L\leq I$. 
Hence,
\begin{align}
\begin{split}
G^{\topp}(I-G)M(I-G)^{\topp}G = G^{\topp}(M-GM)\Minv(M-GM)^{\topp}G &= G^{\topp}M^\half L M^\half G \\
&\leq G^{\topp}MG \\
&\leq G^2
\end{split}
\end{align}
and so
\bes
\lambda_1( G^{\topp}(I-G)M(I-G)^{\topp}G ) \leq \lambda_1(G^2) \leq \gamma_{r,c}.
\ees
In conclusion,
\bes
\rcsqinv \Var(1^{\topp} G^{\topp}(I-G)y) \leq \rcsqinv \gamma_{r,c} \cdot rc = \rcinv \gamma_{r,c} \to 0
\ees
as $r,c \to \infty$. 

Now, $\mu$ is bounded by assumption, while all bounds derived above are independent of $\lambdaa$ and $\lambdab$, therefore $\displaystyle \sup_{|\mu|\leq B; \lambdaa, \lambdab \geq 0} \big\{ \rcsqinv \Var[l_{r,c}(\eta; \etahat^{\mu, \lambdaa, \lambdab})] \big\}$ also tends to zero as $r,c \to \infty$, and (b) is proved.

\eenu

\bigskip
%----------------------------%

\noindent {\it Proof of Theorem~\ref{thm:asym-ol-pr}}. \ 
By definition, $SURE(y; \muhat^{\scriptstyle S}, \lambdaahat^{\scriptstyle S}, \lambdabhat^{\scriptstyle S}) \leq SURE(y; \mutil^{\scriptstyle OL}, \lambdaatil^{\scriptstyle OL}, \lambdabtil^{\scriptstyle OL})$, hence
\bes
P_{r,c} \big\{  L(\eta, \etahat^{\scriptstyle S}) \geq L(\eta, \etatil^{\scriptstyle OL}) + \epsilon \big\} \leq P_{r,c} \big\{  A(y; \eta) \geq B(y; \eta) + \epsilon \big\}
\ees
where
\begin{align*}
A(y; \eta) &= L(\eta, \etahat^{\scriptstyle S}) - SURE(y; \muhat^{\scriptstyle S}, \lambdaahat^{\scriptstyle S}, \lambdabhat^{\scriptstyle S}) \\
B(y; \eta) &= L(\eta, \etatil^{\scriptstyle OL}) - SURE(y; \mutil^{\scriptstyle OL}, \lambdaatil^{\scriptstyle OL}, \lambdabtil^{\scriptstyle OL}).
\end{align*}
Using Markov's inequality and the fact that $A(y; \eta) - B(y; \eta) \geq 0$,
\begin{align*}
P_{r,c} \big\{  A(y; \eta) \geq B(y; \eta) + \epsilon \big\} &\leq \epsilon^{-1} E_{r,c} \{ A(y; \eta) - B(y; \eta) \} \\
&\leq 2 \epsilon^{-1} \sup_{|\mu|\leq B; \ \lambda_1, \lambda_2\geq 0} E_{r,c} | L(\eta, \etahat^{\mu, \lambdaa, \lambdab}) - SURE(y; \mu, \lambdaa, \lambdab) |. 
\end{align*}
Incorporating corollary \eqref{cor:loss-approx}, the last term tends to zero as $r,c \to \infty$. 

\bigskip
%----------------------------%

\noindent {\it Proof of Theorem~\ref{thm:asym-ol-ev}}. \ 
Write
\begin{align*}
L(\eta, \etatil^{\scriptstyle S}) - L(\eta, \etatil^{\scriptstyle OL}) =& \{ L(\eta, \etatil^{\scriptstyle S}) - SURE(y; \muhat^{\scriptstyle S}, \lambdaahat^{\scriptstyle S}, \lambdabhat^{\scriptstyle S}) \} \\
& - \{ L(\eta, \etatil^{\scriptstyle OL}) - SURE(y; \mutil^{\scriptstyle OL}, \lambdaatil^{\scriptstyle OL}, \lambdabtil^{\scriptstyle OL}) \} \\
& + \{ SURE(y; \muhat^{\scriptstyle S}, \lambdaahat^{\scriptstyle S}, \lambdabhat^{\scriptstyle S}) - SURE(y; \mutil^{\scriptstyle OL}, \lambdaatil^{\scriptstyle OL}, \lambdabtil^{\scriptstyle OL}) \}. 
\end{align*}
By definition of $(\muhat^{\scriptstyle S}, \lambdaahat^{\scriptstyle S}, \lambdabhat^{\scriptstyle S})$, the last term is nonpositive, therefore
\begin{align*}
E_{r,c} \{ L(\eta, \etatil^{\scriptstyle S}) - L(\eta, \etatil^{\scriptstyle OL}) \} \leq 
2 \sup_{|\mu|\leq B; \ \lambda_1, \lambda_2\geq 0} E_{r,c} | L(\eta, \etahat^{\mu, \lambdaa, \lambdab}) - SURE(y; \mu, \lambdaa, \lambdab) |
\end{align*}
which tends to zero as $r,c \to \infty$ by Corollary~\ref{cor:loss-approx}. 


\bigskip
%----------------------------%

\noindent {\it Proof of Corollary~\ref{cor:asym-opt}}. \ 
(a) and (b) are direct consequences, respectively, of Theorems ~\ref{thm:asym-ol-pr} and \ref{thm:asym-ol-ev}, since $L(\eta, \etahat^{\muhat, \lambdaahat, \lambdabhat}) \geq L(\eta, \etatil^{\scriptstyle OL})$ and, hence, also $E_{r,c} L(\eta, \etahat^{\muhat, \lambdaahat, \lambdabhat}) \geq E_{r,c} L(\eta, \etatil^{\scriptstyle OL})$. 


\bigskip
\bigskip
%----------------------------%


